Unraveling Consumer Purchase Journey Using Neural Network Models

This study utilizes an ensemble of feedforward neural network models to analyze large-volume and high-dimensional consumer touchpoints and their impact on purchase decisions. When applied to a proprietary dataset of consumer touchpoints and purchases from a global software service provider, the proposed approach demonstrates better predictive accuracy than both traditional models, such as logistic regression, naive Bayes, and k-nearest neighbors, as well as ensemble tree-based classifiers, such as bagging, random forest, AdaBoost, and gradient boosting. By calculating the Shapley values within this network, we provide nuanced insights into touchpoint effectiveness, as we not only assess the marginal impact of diverse touchpoint types but also offer a granular view of the impact distribution within a touchpoint type. Additionally, our model shows excellent adaptability and resilience with limited data resources. When the historical data is reduced from 40 to 1 month, our model shows only a modest 19% decrease in accuracy. This modeling framework can enable managers to more accurately and comprehensively evaluate consumer touchpoints, thereby enhancing the effectiveness and efficiency of their marketing campaigns.

==> Data.tex <==
\section{Data}

Our data is a random sample of $20556$ unique users collected from a multinational digital service provider over the period of 6/1/2018-10/15/2021. For each user, counts for 31 types of marketing touchpoints and purchase information were collected. Descriptions of the marketing touchpoints are in Appendix \ref{sec:appendix}. For the purchase information, users are simply assigned 1 if they purchased any product, and 0 if they did not.

It is of interest not only to predict users' purchase likelihood from the entire $\sim$40-month period of touchpoints but also from shorter interaction periods. In particular, we consider 4 lookback times $T$ ranging from 1 month to the full $\sim$40 months. Table \ref{table:lookbackbuyer} shows the buying likelihood dependent on the lookback. Independent of the lookback, the data is heavily class-imbalanced in that it contains many fewer buyers than non-buyers.

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Lookback length $T$ & 1-month & 3-month & 12-month & Entire period \\
    \hline
    No. of buyers & 2184 & 2263 & 2383 & 2425\\
    \hline
    No. of non-buyers & 17398 & 17670 & 17781 & 18131 \\
    \hline
    Total users & 19582 & 19933 & 20164 & 20556 \\
    \hline
    Buyer percentage & 11.2\% & 11.4\% & 11.8\% & 11.8\% \\
    \hline
\end{tabular}
\caption{Buyer information over different lookback periods.}
\label{table:lookbackbuyer}
\end{table}

The data can be summarized by the input/output pairs
\begin{align}\label{eq:data}
\left\{\mathbf{x}^{(i)}\left[t^{(i)}-T,t^{(i)}\right],y^{(i)}\right\}_{i=1}^{N(T)}
\end{align}
where $N(T)$ is the total number of users (dependent on $T$ as in Table \ref{table:lookbackbuyer}) and $\mathbf{x}\in\mathbb{R}^{31}$ is a 31-dimensional vector of touchpoint counts over the time period $[t(i)-T,t(i)]$ with $T$ the lookback length. If the user is a purchaser, the data collection end time $t(i)$ is the time of purchase (i.e. touchpoints from after the first purchase are not included). If the user is not a purchaser, touchpoint counts from a randomly selected time period of length $T$ are used. A consumer is not included if they are not marketed in the chosen lookback window.
